Audio-Visual Class-Incremental Learning

In this paper, we introduce audio-visual class-incremental learning, a class-incremental learning scenario for audio-visual video recognition. We demonstrate that joint audio-visual modeling can improve class-incremental learning, but current methods fail to preserve semantic similarity between audio and visual features as incremental step grows. Furthermore, we observe that audio-visual correlations learned in previous tasks can be forgotten as incremental steps progress, leading to poor performance. To overcome these challenges, we propose AV-CIL, which incorporates Dual-Audio-Visual Similarity Constraint (D-AVSC) to maintain both instance-aware and class-aware semantic similarity between audio-visual modalities and Visual Attention Distillation (VAD) to retain previously learned audio-guided visual attentive ability. We create three audio-visual class-incremental datasets, AVE-Class-Incremental (AVE-CI), Kinetics-Sounds-Class-Incremental (K-S-CI), and VGGSound100-Class-Incremental (VS100-CI) based on the AVE, Kinetics-Sounds, and VGGSound datasets, respectively. Our experiments on AVE-CI, K-S-CI, and VS100-CI demonstrate that AV-CIL significantly outperforms existing class-incremental learning methods in audio-visual class-incremental learning. Code and data are available at: https://github.com/weiguoPian/AV-CIL_ICCV2023.

==> tables/tb_res_VGG100.tex <==
% \begin{table}[htbp]
\begin{wraptable}{r}{0.25\textwidth}
  \centering
  \caption{Results on VGGSound100-CI.}
    \begin{tabular}{lc}
    \toprule
    Methods & Mean Acc. \\
    \midrule
    % Fine-tuning & 26.21 \\
    SS-IL & 69.20 \\
    AFC-NME & 61.10 \\
    AFC-LSC & 58.15 \\
    \textbf{AV-CIL (ours)} & \textbf{72.80} \\
    % \midrule
    % Oracle (Upper Bound) & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:res_vgg100}%
\end{wraptable} 
% \end{table}%

